A New Re-redistribution Scheme for Weighted State Redistribution with Adaptive Mesh Refinement

State redistribution (SRD) is a recently developed technique for stabilizing cut cells that result from finite-volume embedded boundary methods. SRD has been successfully applied to a variety of compressible and incompressible flow problems. When used in conjunction with adaptive mesh refinement (AMR), additional steps are needed to preserve the accuracy and conservation properties of the solution if the embedded boundary is not restricted to a single level of the mesh hierarchy. In this work, we extend the weighted state redistribution algorithm to cases where cut cells live at or near a coarse-fine interface within the domain. The resulting algorithm maintains conservation and is demonstrated on several two- and three-dimensional example problems.

==> 02_algorithms/redistribution.tex <==
Redistribution is an approach to stabilize cut-cells that arise in finite volume discretization using embedded boundary representations. If we examine the evolution equation \eqref{eq:1d_fv}, we see that the stability of this method requires the time step, $\Delta t$, to be proportional to the cell size, $\Delta x_i$. This creates a prohibitively restrictive requirement on the time step as the size of cut cells can be arbitrarily small. 

==> 02_algorithms/srd_basic.tex <==
% Basic SRD Algorithm - Non-Moving Geometry
We describe here the original state redistribution algorithm (SRD) of Berger and Giuliani \cite{berger2021state} extended to three dimensions. The algorithm comprises a mesh preprocessing step and a solution postprocessing step. After describing these two steps, we will introduce a weighted state redistribution that includes some improvements and generalizations made in \cite{giuliani2022weighted}.
\[\] % Matt - There is probably a better way to do this.
\noindent \textbf{Preprocessing}
\[\] % Matt - There is probably a better way to do this.
Before the time stepping portion of the finite volume solver begins, the mesh is preprocessed by associating a merging neighborhood with each cell in the base grid, both whole and cut.  Small cut cells are merged with their neighbors until the volume of the neighborhood is at least 
$$V_{target} = \Delta x \Delta y \Delta z/2,$$
a threshold informed by results in \cite{berger2015note}. 
This is illustrated in two space dimensions in Figure \ref{fig:cutsWithCounts}a, where cell $(i+1,j-1)$ merges with cell $(i+1,j)$ to form  neighborhood $M_{i+1,j-1}$, highlighted in green.  
Similarly, cell $(i,j-1)$ merges with cell $(i,j)$ to form $M_{i,j-1}$'s neighborhood, shown in Figure \ref{fig:cutsWithCounts}b.
A cell with a volume larger than the threshold value does not merge with any neighboring cells, thus its merging neighborhood only contains itself, like cell $(i,j)$ in Figure \ref{fig:cutsWithCounts}c. Cell $(i+1,j)$ merges with cell $(i,j)$, shown in  Figure \ref{fig:cutsWithCounts}d.

The number of neighborhoods that contain cell $(i,j,k)$, called the overlap count $N_{i,j,k}$, is also indicated in Figure \ref{fig:cutsWithCounts} in two space dimensions.
Cell $(i,j)$ is contained in two other neighborhoods, that of cell $(i,j-1)$ and $(i+1,j)$, plus it is in its own neighborhood by definition, so its overlap count is three (Figure \ref{fig:cutsWithCounts}c). 


There are several possible ways to choose which neighbors a cut cell merges with.  In this example, a cell merges in the direction closest to the boundary normal.  In the AMReX-Hydro implementation, if merging with the one cell in the direction closest to the normal does not result in a neighborhood with a volume greater than $V_{target}$, the neighbor in the direction of the next largest component of the normal is added to the neighborhood.  
In order to not create an ``L-shaped" neighborhood we then automatically add the cell in the same plane as the two neighbors that defines the neighborhood as a 2 $\times$ 2 box.  In 3D if this neighborhood is still not large enough, we then add the remaining four cells to have a 2 $\times$ 2 $\times$ 2 box. 
This is done for aesthetic reasons; an L-shaped domain would still be stable. 
This is illustrated in Figure \ref{fig:3x3}d, where normal merging for cell 9 is insufficient and a larger neighborhood must be used.
This neighborhood is useful in cases where it is desirable to preserve symmetries in the numerical solution, e.g., when the embedded boundary forms exactly a $45^{\circ}$ angle with the background Cartesian grid.

Another alternative is called central merging, where a cut cell is merged with all flow cells that lie on a $3 \times 3 \times 3$ tile centered on that cut cell.  This is neighborhood is larger and more diffusive than normal merging or the 2 $\times$ 2 $\times$ 2 box discussed above.  We will use central merging in some two-dimensional numerical examples (section \ref{sec:ex_2d}).
% In Figure \ref{fig:3x3}, an L-shaped domain is avoided 

In AMReX-Hydro we also made a design decision to preserve spatial symmetries whenever possible. For example, if the boundary normal in a cut cell points has identical components with $n_x = n_y > n_z,$  we create a neighborhood that is larger than strictly necessary on volumetric considerations alone, to avoid directional bias in a possibly otherwise symmetric geometry and solution. 
In the above case the neighborhood would include all fluid cells in a 2 $\times$ 2 $\times$ 1 region in the cut cell's merging neighborhood.  If $n_x = n_y = n_z$ then the neighborhood would include all fluid cells in a 2 $\times$ 2 $\times$ 2 region in the cut cell's merging neighborhood.

 
 Once the neighborhoods have been identified, we define a neighborhood's weighted volume $\widehat V_{i,j,k}$ using the standard cell volume $V_{i,j,k}$ by
 \begin{equation}
\label{eqn:voldef}
{\widehat V}_{i,j,k} =  \sum_{(r,s,t) \in M_{i,j,k} } \,  \frac{V_{r,s,t}}{N_{r,s,t}},
\end{equation}
and a weighted centroid 
\begin{equation}
\label{eqn:centroiddef}
({\widehat x}_{i,j,k},{\widehat y}_{i,j,k},{\widehat z}_{i,j,k}) = \frac{1}{\widehat V_{i,j,k}} \sum_{(r,s,t) \in M_{i,j,k} } \,  \frac{V_{r,s,t}}{N_{r,s,t}}(x_{r,s,t},y_{r,s,t},z_{r,s,t}),
\end{equation}
where $(x_{i,j,k}, y_{i,j,k},z_{i,j,k})$ is the standard cell centroid, and $M_{i,j,k}$ is the set of cells $(r,s,t)$ in the neighborhood of cell $(i,j,k)$.  In the above, cell volumes are weighted by the inverse of their overlap counts.
A cell's overlap count, as well as the weighted volume and centroid associated to neighborhoods are required during the state redistribution postprocessing step, which we describe below.
\[\] % Matt - There is probably a better way to do this.
\noindent \textbf{Postprocessing}
\[\] % Matt - There is probably a better way to do this.
State redistribution is implemented as a postprocessing step acting on cell averages updated by a finite volume scheme. (The finite volume scheme itself needs to be modified for the presence of cut cells to preserve accuracy, but not stability, since that is handled by SRD.) Thus, the first step of the algorithm is to compute a provisional, but possibly unstable cell update
\begin{equation}
% \widehat U_{i,j,k} = U^n_{i,j,k} - \frac{\Delta t}{V_{i,j,k}}\sum_{
% \alpha}  \mathbf{F}_\alpha^*  \cdot \mathbf{n}_\alpha A_\alpha,
\widehat U_{i,j,k} = U^n_{i,j,k} - \frac{\Delta t}{V_{i,j,k}}\sum_{\ell \in \text{faces}}  \mathbf{F}_{\ell}^*  \cdot \mathbf{n}_\ell A_\ell,
\label{eq:eb_update}
\end{equation}
where $A_\ell$ is a face area, $\mathbf{F}_\ell^*$ is the numerical flux, and $\mathbf n_\ell$ is the outward pointing normal.
This update is computed on all cells using a time step $\Delta t$ that is proportional to the size of cells in the background Cartesian grid. 

 The next step is to compute a weighted solution average on each merging neighborhood
 \begin{equation}
 \label{eqn:qhat}
\widehat{Q}_{i,j,k} =  \frac{1}{{\widehat V}_{i,j,k}} \, \sum_{(r,s,t) \in M_{i,j,k}} \,  
\frac{V_{r,s,t}}{N_{r,s,t}}  \widehat{U}_{r,s,t}.
 \end{equation}
For second order accuracy, a gradient is reconstructed in all cells $(i,j,k)$ for which  $M_{i,j,k}$ has at least two cells ($(i,j,k)$ itself and at least one other).
This results in a linear function for neighborhood $(i,j,k)$ of the form
 \begin{equation}\label{eq:qrecon}
\widehat{q}_{i,j,k}(x,y,z) = \widehat{Q}_{i, j,k} + \widehat{\sigma}_{x,i,j,k}(x - \widehat{x}_{i,j,k}) + \widehat{\sigma}_{y,i,j,k}(y - \widehat{y}_{i,j,k}) + \widehat{\sigma}_{z,i,j,k}(z - \widehat{z}_{i,j,k}),
\end{equation}
where $\widehat \sigma$ is the gradient obtained with a least squares approach. 
For this step the least squares equations are  centered on the weighted neighborhood centroids $(\widehat{x}_{i,j,k},\widehat{y}_{i,j,k},\widehat{z}_{i,j,k})$, not the original cell centroids
$(x_{i,j,k},y_{i,j,k},z_{i,j,k})$.

In each coordinate direction, we compute the maximum distance between the weighted centroids of the neighborhoods in the reconstruction stencil to the weighted centroid of the neighborhood on which the reconstruction is centered.
When the reconstruction stencil does not include points further than a threshold in any one coordinate direction, we grow the extent of the stencil in that coordinate direction as described in \cite{BG}.
The threshold distances are defined as $\Delta x/2$, $\Delta y/2$, $\Delta z/2$, in the $x$, $y$, and $z$ directions, respectively.
For example, if the reconstruction stencil is initially the $3\times 3 \times 3$ block, and the maximum distance in the $x$-direction $\max_{m \ne i} |\widehat{x}_i-\widehat{x}_m|$, for cells $m$ in the reconstruction stencil, is not larger than $\Delta x/2$, then the stencil is increased to $5\times 3 \times 3$.
We also point out that the $3 \times 3 \times 3$ block may not contain 27 cells as it could contain covered cells that are not included in the stencil. If the larger stencil still does not contain not enough cells, a well-conditioned gradient reconstruction is not possible, and we drop to first order.

We have also experimented with the less restrictive criterion of requiring the difference between the maximum and minimum centroid values in the stencil to be greater than half the mesh width. More experience in complicated geometries in three dimensions are necessary to ensure this is sufficiently stable.
If necessary, a Barth-Jespersen-style limiting is performed in the neighborhood gradient reconstruction step as well.

The final step is to use the neighborhood polynomial to compute the final solution update
 \begin{equation} \label{eqn:final_update_linear2}
        U^{n+1}_{i,j,k} =   \frac{1}{N_{i,j,k}}\sum_{(r,s,t)  \in W_{i,j,k}}\widehat{q}_{r,s,t}(x_{i,j,k},y_{i,j,k},z_{i,j,k}).
\end{equation}
where $W_{i,j,k}$ is the set of neighborhood indices that include cell $(i,j,k)$ in their neighborhood. 
In words, the stabilized neighborhood solution replaces the unstable finite volume update in a conservative and accurate manner.
In the above formula, the stabilized solution average on a cell in the base grid is obtained by averaging the centroid values of the overlapping merging neighborhood polynomials.  As in the two-dimensional algorithm, SRD can be used with either a method of lines integration in which the SRD algorithm is applied at each stage or with second-order Godunov type approach that directly computes fluxes at the $n+ \frac{1}{2}$ level.

This postprocessing procedure is also applied to the initial data, before any time steps have been taken. This is akin to pre-merging when using cell merging.
It is also analogous to the procedure in incompressible flow, where the initial conditions have an initial projection before time stepping begins.  We have found that our test cases have better monotonicity properties with this additional step.

{\bf Remark:}  This procedure can also be applied to a diffusive flux written in finite volume form. Consider the heat equation $u_t = u_{xx}. $ For this one-dimensional model problem we put one small cut cell at the left boundary of size $\alpha h$ in an otherwise uniform grid with mesh width $h$, as shown in  Figure \ref{fig:1dBndryFig}. 
\begin{figure}[ht!]
    \centering
    \includegraphics[height=.5in]{1dBndryFig.pdf}
    \caption{Notation for 1D model problem with one cut cell at the boundary.}
    \label{fig:1dBndryFig}
\end{figure}
One possible (though not very accurate) finite volume discretization is
\begin{equation}
u_0^{n+1} = u_0^n + \frac{\Delta t}{\alpha h} \left ( \frac{(u_1^n-u_0^n)}{(1+\alpha) h/2} - f_B) \right ) . \label{eq:diff}
\end{equation}
where $f_B$ is a specified boundary flux.
Note that it is $\alpha (1+\alpha)h^2/2 $ and not $(\alpha h)^2$ that appears in the denominator. 
Hence the same SRD procedure that eliminates  $\alpha$ from the denominator for advective updates can be used here too.  As $\alpha \rightarrow 0$, the coefficients of the stabilized finite volume scheme remain bounded. Numerical experiments for this model problem confirm this. A 3D example including a diffusive flux will be presented in sections \ref{sec:compreact} and \ref{sec:compResults}.

==> EB-Flow/cell-unit-square-coord.tex <==
\begin{tikzpicture} [scale=3]

%\draw[white!0] (-0.75,-0.2) rectangle (1.4,1.25);
\draw[white!0] (0.0,-0.4) rectangle (0.1,0.25);
\draw[black] (0.5,0.5) circle [radius=0.5pt];

\coordinate (LL) at (0,0);
\coordinate (UL) at (0,1);
\coordinate (LR) at (1,0);
\coordinate (UR) at (1,1);
%
\coordinate (L1) at (1,0.25);
\coordinate (L2) at (0,0.25);
%
\fill[blue!10] (LL) rectangle (UR);
%
\draw[step=1,gray,very thin] (LL) grid (UR);

\draw[black,-{Triangle[width=5pt,length=5pt]}, line width=0.75pt] (-0.1, 0.5) -- (1.1, 0.5);
\draw[black,-{Triangle[width=5pt,length=5pt]}, line width=0.75pt] (0.5, -0.1) -- (0.5, 1.1);

% Labels
\draw (LL) node [below] {\scriptsize{$(-0.5, -0.5)$}};
\draw (LR) node [below] {\scriptsize{$( 0.5, -0.5)$}};

\draw (UL) node [above] {\scriptsize{$(-0.5,  0.5)$}};
\draw (UR) node [above] {\scriptsize{$( 0.5,  0.5)$}};

\draw (1.1, 0.5) node [right] {\scriptsize{$\xi$}};
\draw (0.5, 1.1) node [above] {\scriptsize{$\eta$}};

\fill[black] (LL)(0,0) circle [radius=0.5pt];
\fill[black] (LR)(1,0) circle [radius=0.5pt];
\fill[black] (UL)(1,1) circle [radius=0.5pt];
\fill[black] (UR)(0,1) circle [radius=0.5pt];

\end{tikzpicture}

==> EB-Flow/eb-flow.tex <==
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{patterns}
\usetikzlibrary{shapes.misc}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{decorations.shapes}

\pgfplotsset{width=10cm,compat=1.9}

\tikzset{cross/.style={%
  cross out, %
  draw=black, %
  minimum size=2*(#1-\pgflinewidth), %
  inner sep=0pt, outer sep=0pt},%
  cross/.default={1pt}%
}


% Partial derivative
\let\oldpartial\partial 
\renewcommand{\partial}[2][]{\dfrac{\oldpartial #1}{\oldpartial #2}}

\begin{comment} % MATT - I put this part into a different file.
This section describes how flow through an embedded boundary surface is captured in the fluid algorithm.

\subsection{Modifications to the convective update}

\subsubsection{Modification to the MAC projection}



Recall that the RHS of the MAC projection is the divergence of the velocity field at face centroids. The contribution of the flow from EB to the RHS is added to the original RHS as follows:

\begin{equation}
    RHS_{i,j,k}^{MAC,total} = RHS_{i,j,k}^{MAC} +
    \frac{1}{\Delta_x V_{i,j,k}} A_{i,j,k}^{EB} (U \cdot \boldsymbol{n})_{i,j,k} 
\end{equation}

where \( A_{i,j,k}^{EB} \) and \( V_{i,j,k} \) are the normalized surface area and volume fractions of the embedded boundary in cell \( (i,j,k) \), respectively.

\subsubsection{Modification to the convective flux}

The convective flux is updated by including the contribution to the divergence as follows:

\begin{equation}
    A_{s,i,j,k}^{\nph,total} = A_{s,i,j,k}^{\nph} +
    \frac{1}{\Delta_x V_{i,j,k}} A_{i,j,k}^{EB} s_{i,j,k}^{\nph}  (U \cdot \boldsymbol{n})_{i,j,k}
\end{equation}


\subsection{Modifications to the diffusive update}
AMReX already includes support for specifying a non-homogeneous Dirichlet boundary condition on the EB surface for the diffusive solver. Hence, the boundary condition for the diffusive solver is modified to impose the flow velocity on the EB surface. No additional implementation was necessary.  

\subsection{Modifications to the nodal projection}
\end{comment}

To compute the approximate projection of the co-located velocity field
$U = (u,v,w)$, we solve the following system for $\phi$. 
\begin{equation}
  D(\beta\nabla\phi) = D(U^{\ast}) - S
  \label{eq:nodal_proj}
\end{equation}
To prepare for the solve, we compute the RHS where the first term
is the divergence of the velocity field at cell nodes. This
is different from the MAC solve where divergence is cell centered and
computed used velocity values at cell faces. 

From the divergence theorem,
\begin{equation} \label{eq:divergence-theorem}
    \int_{\Omega}  U\cdot(\nabla \psi) + \psi(\nabla \cdot U) \; dV = %
       \int_{\oldpartial \Omega}\psi U \cdot\mathbf{n}\; dS
\end{equation}
where $\Omega \subset \mathbb{R}^n$,
$\oldpartial\Omega$ is the boundary of $\Omega$, and
$\mathbf{n}(\mathbf{r})$ is the outward facing unit vector to the surface $\oldpartial\Omega$ 
at point $\mathbf{r}\in\oldpartial\Omega$. %
%
Rewriting, we obtain
\begin{equation} \label{eq:divergence-theorem:weak-form}
    \int_{\Omega}  \psi(\nabla \cdot U) \; dV = %
    -\int_{\Omega} U\cdot(\nabla \psi) \; dV + %
       \int_{\oldpartial \Omega}\psi U\cdot\mathbf{n}\; dS
\end{equation}
We want to approach this from a finite-element perspective, thinking
of $\psi$ as basis functions. Additionally, we want to limit our attention
to the unit square whose low and high side faces are at $-0.5$ and $0.5$,
respectively.
Figure \ref{fig:mapping:cell:physical-space} depicts the mapping of cell $(i,j)$ to
the unit square in $(\xi, \eta)$ space with the same node ordering. Because
\texttt{AMReX} is based on block-structured meshes, these notes may
drop $j$ indices from $x$-coordinates and $i$ indices from $y$-coordinates
to simplify the notation when no confusion will arise.


\begin{figure}[ht!]
  \captionsetup[sub]{justification=centering}
  \centering
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \input{EB-Flow/nodal-mapping}
    \caption{ }
    \label{fig:mapping:cell:physical-space}
  \end{subfigure}
  \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \input{EB-Flow/cell-unit-square-coord}
    \caption{ }
    \label{fig:mapping:cell:computational-space}
  \end{subfigure}
  \caption{Illustration of mapping from physical cell to unit square.}
%  \label{fig:mapping:cells}
  \label{fig:mapping}
\end{figure}

To make things a little more concrete, consider node $(i,j)$ illustrated 
in Figure \ref{fig:mapping:cell:physical-space} and the four adjacent cells:
$(i,j)$, $(i-1,j)$, $(i-1,j-1)$, and $(i,j-1)$, where the cell and node indexing
is consistent with \texttt{AMReX}. The divergence we compute at this node
has contributions from each of the adjacent cells. First, let's focus
on cell $(i,j)$ in the upper, right corner that is shaded blue. We want
to construct a basis function that is 1 at node $(i,j)$ and 0 at the other nodes.
To this end, we choose the simple bilinear function,
\begin{equation*}
    \psi_{i,j,k}(x,y,z) = 
    \begin{cases} 
        \frac{x_{i+1} - x}{x_{i+1} - x_i}
        \frac{y_{j+1} - y}{y_{j+1} - y_j}
        \frac{z_{k+1} - y}{z_{k+1} - z_j}
        & \text{for\;\;} x\in [x_{i},x_{i+1}] \land
                         y\in [y_{j},y_{j+1}] \land
                         z\in [z_{k},z_{k+1}] \\
        0  & \text{otherwise}
   \end{cases} 
\end{equation*}
Because we use a uniform mesh,%
\footnote{On a single level, all meshes are the same $\Delta_x$, $\Delta_y$, and $\Delta_z$} %
we can define
$\Delta_x = x_{i+1}-x_i$ for all $i$ and 
$\Delta_y = y_{j+1}-y_j$ for all $j$ and
$\Delta_z = z_{k+1}-z_k$ for all $k$ such that
$x_{i+1} = x_i + \Delta_x$,
$y_j = y_j + \Delta_j$, and
$z_k = z_k + \Delta_k$.
These definitions allow us to rewrite the basis function as 
\begin{equation}
    \psi_{i,j,k}(\xi,\eta,\zeta) = 
    \begin{cases} 
        \left(\frac{1}{2} - \xi(x)\right)%
        \left(\frac{1}{2} - \eta(y)\right)%
        \left(\frac{1}{2} - \zeta(z)\right)%
        & \text{for\;\;} \xi,\eta, \zeta \in [-1/2, 1/2] \\
        0  & \text{otherwise}
   \end{cases} 
\end{equation}
where
\begin{equation} \label{eq:mapping:cell:ij}
   \xi_i(x)   = \left(\frac{x - x_i}{\Delta_x} - \frac{1}{2}\right), \quad
   \eta_j(y)  = \left(\frac{y - y_j}{\Delta_y} - \frac{1}{2}\right), \quad\text{and}\quad
   \zeta_k(z) = \left(\frac{z - z_k}{\Delta_z} - \frac{1}{2}\right).
\end{equation}
Note that $\xi_i(x)$, $\eta_j(y)$ and $\zeta_k(z)$ achieve the desired mapping
from physical coordinates to the unit cube. Each cell in the
in the neighborhood for node $(i,j,k)$ has a different basis
function, but still results in mapping to the unit cube.
\begin{align*}
    \psi_{i,j,k\phantom{-1-1-1}}   &= (1/2 - \xi) ( 1/2 - \eta) ( 1/2 - \zeta) \\%
    \psi_{i-1,j,k\phantom{-1-1}}   &= (1/2 + \xi) ( 1/2 - \eta) ( 1/2 - \zeta) \\%
    \psi_{i,j-1,k\phantom{-1-1}}   &= (1/2 - \xi) ( 1/2 + \eta) ( 1/2 - \zeta) \\%
    \psi_{i-1,j-1,k\phantom{-1}}   &= (1/2 + \xi) ( 1/2 + \eta) ( 1/2 - \zeta) \\%
    \psi_{i,j,k-1\phantom{-1-1}}   &= (1/2 - \xi) ( 1/2 - \eta) ( 1/2 + \zeta) \\%
    \psi_{i-1,j,k-1\phantom{-1}}   &= (1/2 + \xi) ( 1/2 - \eta) ( 1/2 + \zeta) \\%
    \psi_{i,j-1,k-1\phantom{-1}}   &= (1/2 - \xi) ( 1/2 + \eta) ( 1/2 + \zeta) \\%
    \psi_{i-1,j-1,k-1}             &= (1/2 + \xi) ( 1/2 + \eta) ( 1/2 + \zeta) \\%
\end{align*}
We need to observation that
\begin{equation} \label{eq:mapping:partials}
   \partial[\psi]x = \partial[\psi]\xi   \partial[\xi  ]x, \quad
   \partial[\psi]y = \partial[\psi]\eta  \partial[\eta ]y, \quad\text{and}\quad
   \partial[\psi]z = \partial[\psi]\zeta \partial[\zeta]z
\end{equation}
where $\oldpartial\xi/\oldpartial x = 1/\Delta_x$,
$\oldpartial\eta/\oldpartial y = 1/\Delta_y$, and
$\oldpartial\zeta/\oldpartial z = 1/\Delta_z$
are obtained from Eq.~\eqref{eq:mapping:cell:ij}.



\subsubsection{Computing $D(U)$ for node $(i,j,k)$}

Turning our attention back to Eq.~\eqref{eq:divergence-theorem:weak-form}, we can write the
RHS as the sum of the contributions from the adjacent cells.
%\begin{equation*}
%\begin{split}
%    -\int_{\Omega} U\cdot(\nabla \psi) \; dV \approx
%     -\int_{\Omega_{i,j}} U_{i  ,j  }\cdot(\nabla \psi_{i  ,j  }) \; dV
%       + \int_{\oldpartial \Omega_{i  ,j  }}\psi_{i  ,j  } U_{i  ,j  }\cdot\mathbf{n}\; dS \\
%     -\int_{\Omega_{i,j}} U_{i-1,j  }\cdot(\nabla \psi_{i-1,j  }) \; dV 
%       + \int_{\oldpartial \Omega_{i-1,j  }}\psi_{i-1,j  } U_{i-1,j  }\cdot\mathbf{n}\; dS \\
%     -\int_{\Omega_{i,j}} U_{i-1,j-1}\cdot(\nabla \psi_{i-1,j-1}) \; dV
%       + \int_{\oldpartial \Omega_{i-1,j-1}}\psi_{i-1,j-1} U_{i-1,j-1}\cdot\mathbf{n}\; dS \\
%     -\int_{\Omega_{i,j}} U_{i  ,j-1}\cdot(\nabla \psi_{i  ,j-1}) \; dV
%       + \int_{\oldpartial \Omega_{i  ,j-1}}\psi_{i  ,j-1} U_{i  ,j-1}\cdot\mathbf{n}\; dS \\
%\end{split}
%\end{equation*}
%
For each cell, we will look at the volume integral, $-\int_{\Omega}U\cdot\nabla\phi dV$,
and surface integral, $U_{eb} = U_{i,j,k} \cdot \mathbf{n}$, separately. 
This will allow us to better understand how \texttt{AMReX} currently calculates
the nodal divergence, where the contribution from the EB is assumed zero,
and what modifications we need to make.

\paragraph{2D}\mbox{} \\
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                       (i,j)                                          %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Starting with cell $(i,j)$, the basis function its gradient are
\begin{equation*}
    \psi_{i  ,j } = (0.5 - \xi)(0.5 - \eta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i  ,j  ,k  } = ( 
       -(0.5 - \eta)(0.5 - \zeta)/\Delta_x, 
       -(0.5 - \xi )(0.5 - \zeta)/\Delta_y ),
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i  ,j  }^E} U_{i  ,j }&\cdot(\nabla \psi_{i  ,j}) \; dxdy \\
%
       &=
                    - U_x\int_{\Omega_{i  ,j }^0} -(0.5 - \eta)/\Delta_x \; d\xi d\eta \\
       &\phantom{=} - U_y\int_{\Omega_{i  ,j }^0} -(0.5 - \xi )(0.5 - \zeta)/\Delta_y \\
       &\phantom{=} - U_v\int_{\Omega_{i  ,j  ,k  }^0} -(0.5 - \xi )(0.5 - \eta )/\Delta_z \\
%
       &=
           0.5/\Delta_x \, U_x (\Lambda - 2S_y) + 0.5/\Delta_y \, U_y (\Lambda - 2S_x)  \\
\end{align*}

where we've adopted the notation \( \Lambda = \int 1 \; d\xi d\eta \), \(S_x = \int \xi \; d\xi d\eta \), and \(S_y = \int \eta \; d\xi d\eta \) are fully defined later.
%
%
Now let's look at the contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i  ,j}^E}&\psi_{i  ,j } \left(U_{i  ,j}\cdot \mathbf{n}_{i  ,j}\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i  ,j}
           \int_{\oldpartial\Omega^0} (0.5 - \xi)(0.5 - \eta)\; ds \\
%
       &= 0.25 \left(U\cdot \mathbf{n}\right)_{i  ,j}
           \int_{\oldpartial\Omega^0} (
           1 - 2\xi - 2\eta + 4\xi\eta) \; ds \\
%
       &= 0.25 \left(U\cdot \mathbf{n}\right)_{i  ,j } \left(
          A_{EB} - 2 B_x - 2 B_y + 4 B_{xy} \right) .\\
\end{align*}

where we've adopted the notation \(A_{EB} = \int_{\oldpartial\Omega^0} 1 \; ds \), \( B_x = \int_{\oldpartial\Omega^0} \xi \; ds \), \( B_y = \int_{\oldpartial\Omega^0} \eta \; ds \), and \( B_{xy} = \int_{\oldpartial\Omega^0} \xi \eta \; ds \) to be defined later. Observe that the integration remains over the unit square so that the parametrization has yet to be determined.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                      (i-1,j)                                         %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent Moving to cell $(i-1,j)$, the basis function and its gradient are
\begin{equation*}
    \psi_{i-1,j} = (0.5 + \xi)(0.5 - \eta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i-1,j} = ( 
        (0.5 - \eta)/\Delta_x, 
       -(0.5 + \xi )/\Delta_y,
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i-1,j}^E} U_{i-1,j}&\cdot(\nabla \psi_{i-1,j}) \; dxdy \\
%
       &=
                    - U_x\int_{\Omega_{i-1,j}^0}  (0.5 - \eta)/\Delta_x \; d\xi d\eta \\
       &\phantom{=} - U_y\int_{\Omega_{i-1,j}^0} -(0.5 + \xi )/\Delta_y \; d\xi d\eta \\
       &=
         - 0.5/\Delta_x \, U_x (\Lambda - 2S_y)  + 0.5/\Delta_y \, U_y (\Lambda + 2S_x)  \\
\end{align*}

Looking at the contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i-1,j}^E}&\psi_{i-1,j} \left(U_{i-1,j}\cdot \mathbf{n}_{i-1,j}\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i-1,j}
           \int_{\oldpartial\Omega^0} (0.5 + \xi)(0.5 - \eta) \; ds \\
%
       &= 0.25 \left(U\cdot \mathbf{n}\right)_{i-1,j  ,k  }
           \int_{\oldpartial\Omega^0} (
           1 + 2\xi - 2\eta - 4\xi\eta) \; ds \\
%
       &= 0.25 \left(U\cdot \mathbf{n}\right)_{i-1,j  ,k  } \left(
          A_{EB} + 2 B_x - 2 B_y - 4 B_{xy} \right) .\\
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                     (i-1,j-1)                                        %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent For cell $(i-1,j-1)$, the basis function is
\begin{equation*}
    \psi_{i-1,j-1,k  } = (0.5 + \xi)(0.5 + \eta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i-1,j-1} = ( 
        (0.5 + \eta)/\Delta_x, 
        (0.5 + \xi )/\Delta_y)
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i-1,j-1}^E} U_{i-1,j-1}&\cdot(\nabla \psi_{i-1,j-1}) \; dxdy \\
%
       &=
                    - U_x\int_{\Omega_{i-1,j-1}^0}  (0.5 + \eta)/\Delta_x \; d\xi d\eta \\
       &\phantom{=} - U_y\int_{\Omega_{i-1,j-1}^0}  (0.5 + \xi )/\Delta_y \; d\xi d\eta \\
       &=
         - 0.5/\Delta_x \, U_x (\Lambda + 2S_y - 2S_z) - 0.5/\Delta_y \, U_y (\Lambda + 2S_x - 2S_z)  \\
\end{align*}

The contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i-1,j-1}^E}&\psi_{i-1,j-1} \left(U_{i-1,j-1}\cdot \mathbf{n}_{i-1,j-1}\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i-1,j-1}
           \int_{\oldpartial\Omega^0} (0.5 + \xi)(0.5 + \eta) \; ds \\
%
       &= 0.25 \left(U\cdot \mathbf{n}\right)_{i-1,j-1}
           \int_{\oldpartial\Omega^0} (
           1 + 2\xi + 2\eta + 4\xi\eta ) \; ds \\
%
       &= 0.25 \left(U\cdot \mathbf{n}\right)_{i-1,j-1} \left(
          A_{EB} + 2 B_x + 2 B_y + 4 B_{xy} \right) .\\
\end{align*}
%
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                      (i,j-1)                                         %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent Finally for cell $(i,j-1)$ the basis function and its gradient are
\begin{equation*}
    \psi_{i  ,j-1} = (0.5 - \xi)(0.5 + \eta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i  ,j-1} = ( 
       -(0.5 + \eta)/\Delta_x, 
        (0.5 - \xi )/\Delta_y)
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i  ,j  }^E} U_{i  ,j-1}&\cdot(\nabla \psi_{i  ,j-1}) \; dxdy \\
%
       &=
                    - U_x\int_{\Omega_{i  ,j-1,k  }^0} -(0.5 + \eta)/\Delta_x \; d\xi d\eta \\
       &\phantom{=} - U_y\int_{\Omega_{i  ,j-1}^0}  (0.5 - \xi )/\Delta_y \; d\xi d\eta \\
       &=
           0.5/\Delta_x \, U_x (\Lambda + 2S_y) - 0.5/\Delta_y \, U_y (\Lambda - 2S_x) 
\end{align*}

The contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i  ,j-1}^E}&\psi_{i  ,j-1} \left(U_{i  ,j-1}\cdot \mathbf{n}_{i  ,j-1}\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i  ,j-1}
           \int_{\oldpartial\Omega^0} (0.5 - \xi)(0.5 + \eta) \; ds \\
%
       &= 0.25 \left(U\cdot \mathbf{n}\right)_{i  ,j-1}
           \int_{\oldpartial\Omega^0} (
           1 - 2\xi + 2\eta - 4\xi\eta ) \; ds \\
%
       &= 0.25 \left(U\cdot \mathbf{n}\right)_{i  ,j-1} \left(
          A_{EB} - 2 B_x + 2 B_y - 4 B_{xy} \right) .\\
\end{align*}
%
%

\noindent Summing all the terms, we get
\begin{equation*}
\begin{split}
     -\int U \cdot(\nabla \psi) \; dV  &= 
    -\int_{\Omega} U\cdot(\nabla \psi) \; dV + %
       \int_{\oldpartial \Omega}\psi U\cdot\mathbf{n}\; dS =  \\
%
      0.5/\Delta_x \Big( &u_{i-1,j-1 } ( -\Lambda - 2S_y)  \\
                      +  &u_{i  ,j-1 \phantom{   -1}} ( +\Lambda + 2S_y)  \\
                      +  &u_{i-1,j   \phantom{   -1}} ( -\Lambda + 2S_y)  \\
                      +  &u_{i  ,j   \phantom{ -1-1}} ( +\Lambda - 2S_y)
                   \Big) \\
    + 0.5/\Delta_y \Big( &v_{i-1,j-1 } ( -\Lambda - 2S_x)  \\
                      +  &v_{i  ,j-1 \phantom{   -1}} ( -\Lambda + 2S_x)  \\
                      +  &v_{i-1,j   \phantom{   -1}} ( +\Lambda + 2S_x)  \\
                      +  &v_{i  ,j   \phantom{ -1-1}} ( +\Lambda - 2S_x) 
                    \Big) \\
    + 0.25 \Big(
               &\left(U\cdot \mathbf{n}\right)_{i-1,j-1 \phantom{    -1}}
                   \left( A_{EB} + 2 B_x + 2 B_y + 4 B_{xy} \right) \\
            +  &\left(U\cdot \mathbf{n}\right)_{i  ,j-1 \phantom{-1  -1}}
                   \left( A_{EB} - 2 B_x + 2 B_y - 4 B_{xy} \right) \\
            +  &\left(U\cdot \mathbf{n}\right)_{i-1,j  \phantom{  -1-1}}
                   \left( A_{EB} + 2 B_x - 2 B_y - 4 B_{xy} \right) \\
            +  &\left(U\cdot \mathbf{n}\right)_{i  ,j  \phantom{-1-1-1}}
                   \left( A_{EB} - 2 B_x - 2 B_y + 4 B_{xy} \right)
           \Big)
\end{split}
\end{equation*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%               3D
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{3D}\mbox \\
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                       (i,j,k)                                          %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Starting with cell $(i,j,k)$, the basis function its gradient are
\begin{equation*}
    \psi_{i  ,j  ,k  } = (0.5 - \xi)(0.5 - \eta)(0.5 - \zeta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i  ,j  ,k  } = ( 
       -(0.5 - \eta)(0.5 - \zeta)/\Delta_x, 
       -(0.5 - \xi )(0.5 - \zeta)/\Delta_y,
       -(0.5 - \xi )(0.5 - \eta )/\Delta_z ),
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i  ,j  }^E} U_{i  ,j  ,k  }&\cdot(\nabla \psi_{i  ,j  ,k  }) \; dxdydz \\
%
       &=
                    - U_x\int_{\Omega_{i  ,j  ,k  }^0} -(0.5 - \eta)(0.5 - \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_y\int_{\Omega_{i  ,j  ,k  }^0} -(0.5 - \xi )(0.5 - \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_v\int_{\Omega_{i  ,j  ,k  }^0} -(0.5 - \xi )(0.5 - \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%
       &=
           0.25/\Delta_x \, U_x (\Lambda - 2S_y - 2S_z + 4S_{yz})  \\
       & + 0.25/\Delta_y \, U_y (\Lambda - 2S_x - 2S_z + 4S_{xz})  \\
       & + 0.25/\Delta_z \, U_z (\Lambda - 2S_x - 2S_y + 4S_{xy})  \\
\end{align*}
%
%
Now let's look at the contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i  ,j  ,k  }^E}&\psi_{i  ,j  ,k  } \left(U_{i  ,j  ,k  }\cdot \mathbf{n}_{i  ,j  ,k  }\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i  ,j  ,k  }
           \int_{\oldpartial\Omega^0} (0.5 - \xi)(0.5 - \eta)(0.5 - \zeta) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i  ,j  ,k  }
           \int_{\oldpartial\Omega^0} (
           1 - 2\xi - 2\eta + 4\xi\eta - 2\zeta + 4\eta\zeta + 4\xi\zeta - 8 \xi\eta\zeta ) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i  ,j  ,k  } \left(
          A_{EB} - 2 B_x - 2 B_y + 4 B_{xy} - 2 B_z + 4 B_{yz} + 4 B_{xz} - 8 B_{xyz} \right) .\\
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                      (i-1,j,k)                                         %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent Moving to cell $(i-1,j  ,k  )$, the basis function and its gradient are
\begin{equation*}
    \psi_{i-1,j  ,k  } = (0.5 + \xi)(0.5 - \eta)(0.5 - \zeta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i-1,j  ,k  } = ( 
        (0.5 - \eta)(0.5 - \zeta)/\Delta_x, 
       -(0.5 + \xi )(0.5 - \zeta)/\Delta_y,
       -(0.5 + \xi )(0.5 - \eta )/\Delta_z ),
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i-1,j  ,k  }^E} U_{i-1,j  ,k  }&\cdot(\nabla \psi_{i-1,j  ,k  }) \; dxdydz \\
%
       &=
                    - U_x\int_{\Omega_{i-1,j  ,k  }^0}  (0.5 - \eta)(0.5 - \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_y\int_{\Omega_{i-1,j  ,k  }^0} -(0.5 + \xi )(0.5 - \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_v\int_{\Omega_{i-1,j  ,k  }^0} -(0.5 + \xi )(0.5 - \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    - U_x\int_{\Omega_{i-1,j  ,k  }^0}  (0.5 - \eta)(0.5 - \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_y\int_{\Omega_{i-1,j  ,k  }^0}  (0.5 + \xi )(0.5 - \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_v\int_{\Omega_{i-1,j  ,k  }^0}  (0.5 + \xi )(0.5 - \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    - U_x\int_{\Omega_{i-1,j  ,k  }^0}  (0.25 - 0.5\eta - 0.5\zeta + \eta\zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_y\int_{\Omega_{i-1,j  ,k  }^0}  (0.25 + 0.5\xi  - 0.5\zeta - \xi \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_v\int_{\Omega_{i-1,j  ,k  }^0}  (0.25 + 0.5\xi  - 0.5\eta  - \xi \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%
       &=
         - 0.25/\Delta_x \, U_x (\Lambda - 2S_y - 2S_z + 4S_{yz})  \\
       & + 0.25/\Delta_y \, U_y (\Lambda + 2S_x - 2S_z - 4S_{xz})  \\
       & + 0.25/\Delta_z \, U_z (\Lambda + 2S_x - 2S_y - 4S_{xy})  \\
\end{align*}

Looking at the contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i-1,j  ,k  }^E}&\psi_{i-1,j  ,k  } \left(U_{i-1,j  ,k  }\cdot \mathbf{n}_{i-1,j  ,k  }\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i-1,j  ,k  }
           \int_{\oldpartial\Omega^0} (0.5 + \xi)(0.5 - \eta)(0.5 - \zeta) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i-1,j  ,k  }
           \int_{\oldpartial\Omega^0} (
           1 + 2\xi - 2\eta - 4\xi\eta - 2\zeta + 4\eta\zeta - 4\xi\zeta +8 \xi\eta\zeta ) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i-1,j  ,k  } \left(
          A_{EB} + 2 B_x - 2 B_y - 4 B_{xy} - 2 B_z + 4 B_{yz} - 4 B_{xz} + 8 B_{xyz} \right) .\\
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                      (i,j-1,k)                                         %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent For cell $(i,j-1,k)$ the basis function and its gradient are
\begin{equation*}
    \psi_{i  ,j-1,k  } = (0.5 - \xi)(0.5 + \eta)(0.5 - \zeta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i  ,j-1,k  } = ( 
       -(0.5 + \eta)(0.5 - \zeta)/\Delta_x, 
        (0.5 - \xi )(0.5 - \zeta)/\Delta_y,
       -(0.5 - \xi )(0.5 + \eta )/\Delta_z ),
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i  ,j  }^E} U_{i  ,j-1,k  }&\cdot(\nabla \psi_{i  ,j-1,k  }) \; dxdydz \\
%
       &=
                    - U_x\int_{\Omega_{i  ,j-1,k  }^0} -(0.5 + \eta)(0.5 - \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_y\int_{\Omega_{i  ,j-1,k  }^0}  (0.5 - \xi )(0.5 - \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_v\int_{\Omega_{i  ,j-1,k  }^0} -(0.5 - \xi )(0.5 + \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    + U_x\int_{\Omega_{i  ,j-1,k  }^0}  (0.5 + \eta)(0.5 - \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_y\int_{\Omega_{i  ,j-1,k  }^0}  (0.5 - \xi )(0.5 - \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_v\int_{\Omega_{i  ,j-1,k  }^0}  (0.5 - \xi )(0.5 + \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    + U_x\int_{\Omega_{i  ,j-1,k  }^0}  (0.25 + 0.5\eta - 0.5\zeta - \eta\zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_y\int_{\Omega_{i  ,j-1,k  }^0}  (0.25 - 0.5\xi  - 0.5\zeta + \xi \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_v\int_{\Omega_{i  ,j-1,k  }^0}  (0.25 - 0.5\xi  + 0.5\eta  - \xi \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%
       &=
           0.25/\Delta_x \, U_x (\Lambda + 2S_y - 2S_z - 4S_{yz})  \\
       & - 0.25/\Delta_y \, U_y (\Lambda - 2S_x - 2S_z + 4S_{xz})  \\
       & + 0.25/\Delta_z \, U_z (\Lambda - 2S_x + 2S_y - 4S_{xy})  \\
\end{align*}

The contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i  ,j-1,k  }^E}&\psi_{i  ,j-1,k  } \left(U_{i  ,j-1,k  }\cdot \mathbf{n}_{i  ,j-1,k  }\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i  ,j-1,k  }
           \int_{\oldpartial\Omega^0} (0.5 - \xi)(0.5 + \eta)(0.5 - \zeta) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i  ,j-1,k  }
           \int_{\oldpartial\Omega^0} (
           1 - 2\xi + 2\eta - 4\xi\eta - 2\zeta - 4\eta\zeta + 4\xi\zeta + 8 \xi\eta\zeta ) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i  ,j-1,k  } \left(
          A_{EB} - 2 B_x + 2 B_y - 4 B_{xy} - 2 B_z - 4 B_{yz} + 4 B_{xz} + 8 B_{xyz} \right) .\\
\end{align*}
%
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                     (i-1,j-1,k)                                        %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent For cell $(i-1,j-1,k)$, the basis function is
\begin{equation*}
    \psi_{i-1,j-1,k  } = (0.5 + \xi)(0.5 + \eta)(0.5 - \zeta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i-1,j-1,k  } = ( 
        (0.5 + \eta)(0.5 - \zeta)/\Delta_x, 
        (0.5 + \xi )(0.5 - \zeta)/\Delta_y,
       -(0.5 + \xi )(0.5 + \eta )/\Delta_z ),
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i-1,j-1,k  }^E} U_{i-1,j-1,k  }&\cdot(\nabla \psi_{i-1,j-1,k  }) \; dxdydz \\
%
       &=
                    - U_x\int_{\Omega_{i-1,j-1,k  }^0}  (0.5 + \eta)(0.5 - \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_y\int_{\Omega_{i-1,j-1,k  }^0}  (0.5 + \xi )(0.5 - \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_v\int_{\Omega_{i-1,j-1,k  }^0} -(0.5 + \xi )(0.5 + \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    - U_x\int_{\Omega_{i-1,j-1,k  }^0}  (0.5 + \eta)(0.5 - \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_y\int_{\Omega_{i-1,j-1,k  }^0}  (0.5 + \xi )(0.5 - \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_v\int_{\Omega_{i-1,j-1,k  }^0}  (0.5 + \xi )(0.5 + \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    - U_x\int_{\Omega_{i-1,j-1,k  }^0}  (0.25 + 0.5\eta - 0.5\zeta - \eta\zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_y\int_{\Omega_{i-1,j-1,k  }^0}  (0.25 + 0.5\xi  - 0.5\zeta - \xi \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_v\int_{\Omega_{i-1,j-1,k  }^0}  (0.25 + 0.5\xi  + 0.5\eta  + \xi \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%
       &=
         - 0.25/\Delta_x \, U_x (\Lambda + 2S_y - 2S_z - 4S_{yz})  \\
       & - 0.25/\Delta_y \, U_y (\Lambda + 2S_x - 2S_z - 4S_{xz})  \\
       & + 0.25/\Delta_z \, U_z (\Lambda + 2S_x + 2S_y + 4S_{xy})  \\
\end{align*}

The contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i-1,j-1,k  }^E}&\psi_{i-1,j-1,k  } \left(U_{i-1,j-1,k  }\cdot \mathbf{n}_{i-1,j-1,k  }\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i-1,j-1,k  }
           \int_{\oldpartial\Omega^0} (0.5 + \xi)(0.5 + \eta)(0.5 - \zeta) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i-1,j-1,k  }
           \int_{\oldpartial\Omega^0} (
           1 + 2\xi + 2\eta + 4\xi\eta - 2\zeta - 4\eta\zeta - 4\xi\zeta - 8 \xi\eta\zeta ) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i-1,j-1,k  } \left(
          A_{EB} + 2 B_x + 2 B_y + 4 B_{xy} - 2 B_z - 4 B_{yz} - 4 B_{xz} - 8 B_{xyz} \right) .\\
\end{align*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                        (i,j,k-1)                                       %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent For cell $(i  ,j  ,k-1)$, the basis function and its gradient are
\begin{equation*}
    \psi_{i  ,j  ,k-1} = (0.5 - \xi)(0.5 - \eta)(0.5 + \zeta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i  ,j  ,k-1} = ( 
       -(0.5 - \eta)(0.5 + \zeta)/\Delta_x, 
       -(0.5 - \xi )(0.5 + \zeta)/\Delta_y,
        (0.5 - \xi )(0.5 - \eta )/\Delta_z ),
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i  ,j  }^E} U_{i  ,j  ,k-1}&\cdot(\nabla \psi_{i  ,j  ,k-1}) \; dxdydz \\
%
       &=
                    - U_x\int_{\Omega_{i  ,j  ,k-1}^0} -(0.5 - \eta)(0.5 + \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_y\int_{\Omega_{i  ,j  ,k-1}^0} -(0.5 - \xi )(0.5 + \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_v\int_{\Omega_{i  ,j  ,k-1}^0}  (0.5 - \xi )(0.5 - \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                      U_x\int_{\Omega_{i  ,j  ,k-1}^0}  (0.5 - \eta)(0.5 + \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_y\int_{\Omega_{i  ,j  ,k-1}^0}  (0.5 - \xi )(0.5 + \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_v\int_{\Omega_{i  ,j  ,k-1}^0}  (0.5 - \xi )(0.5 - \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                      U_x\int_{\Omega_{i  ,j  ,k-1}^0}  (0.25 - 0.5\eta + 0.5\zeta - \eta\zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_y\int_{\Omega_{i  ,j  ,k-1}^0}  (0.25 - 0.5\xi  + 0.5\zeta - \xi \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_v\int_{\Omega_{i  ,j  ,k-1}^0}  (0.25 - 0.5\xi  - 0.5\eta  + \xi \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%
       &=
           0.25/\Delta_x \, U_x (\Lambda - 2S_y + 2S_z - 4S_{yz})  \\
       & + 0.25/\Delta_y \, U_y (\Lambda - 2S_x + 2S_z - 4S_{xz})  \\
       & - 0.25/\Delta_z \, U_z (\Lambda - 2S_x - 2S_y + 4S_{xy})  \\
\end{align*}
\begin{align*}
     \int_{\oldpartial\Omega_{i  ,j  ,k-1}^E}&\psi_{i  ,j  ,k-1} \left(U_{i  ,j  ,k-1}\cdot \mathbf{n}_{i  ,j  ,k-1}\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i  ,j  ,k-1}
           \int_{\oldpartial\Omega^0} (0.5 - \xi)(0.5 - \eta)(0.5 + \zeta) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i  ,j  ,k-1}
           \int_{\oldpartial\Omega^0} (
           1 - 2\xi - 2\eta + 4\xi\eta + 2\zeta - 4\eta\zeta - 4\xi\zeta + 8 \xi\eta\zeta ) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i  ,j  ,k-1} \left(
          A_{EB} - 2 B_x - 2 B_y + 4 B_{xy} + 2 B_z - 4 B_{yz} - 4 B_{xz} + 8 B_{xyz} \right) .\\
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                       (i-1,j,k-1)                                      %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent For cell $(i-1,j  ,k-1)$, the basis function and its gradient are
\begin{equation*}
    \psi_{i-1,j  ,k-1} = (0.5 + \xi)(0.5 - \eta)(0.5 + \zeta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i-1,j  ,k-1} = ( 
        (0.5 - \eta)(0.5 + \zeta)/\Delta_x, 
       -(0.5 + \xi )(0.5 + \zeta)/\Delta_y,
        (0.5 + \xi )(0.5 - \eta )/\Delta_z ),
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i-1,j  }^E} U_{i-1,j  ,k-1}&\cdot(\nabla \psi_{i-1,j  ,k-1}) \; dxdydz \\
%
       &=
                    - U_x\int_{\Omega_{i-1,j  ,k-1}^0}  (0.5 - \eta)(0.5 + \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_y\int_{\Omega_{i-1,j  ,k-1}^0} -(0.5 + \xi )(0.5 + \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_v\int_{\Omega_{i-1,j  ,k-1}^0}  (0.5 + \xi )(0.5 - \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    - U_x\int_{\Omega_{i-1,j  ,k-1}^0}  (0.5 - \eta)(0.5 + \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_y\int_{\Omega_{i-1,j  ,k-1}^0}  (0.5 + \xi )(0.5 + \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_v\int_{\Omega_{i-1,j  ,k-1}^0}  (0.5 + \xi )(0.5 - \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    - U_x\int_{\Omega_{i-1,j  ,k-1}^0}  (0.25 - 0.5\eta + 0.5\zeta - \eta\zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} + U_y\int_{\Omega_{i-1,j  ,k-1}^0}  (0.25 + 0.5\xi  + 0.5\zeta + \xi \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_v\int_{\Omega_{i-1,j  ,k-1}^0}  (0.25 + 0.5\xi  - 0.5\eta  - \xi \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%
       &=
         - 0.25/\Delta_x \, U_x (\Lambda - 2S_y + 2S_z - 4S_{yz})  \\
       & + 0.25/\Delta_y \, U_y (\Lambda + 2S_x + 2S_z + 4S_{xz})  \\
       & - 0.25/\Delta_z \, U_z (\Lambda + 2S_x - 2S_y - 4S_{xy})  \\
\end{align*}
The contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i-1,j  ,k-1}^E}&\psi_{i-1,j  ,k-1} \left(U_{i-1,j  ,k-1}\cdot \mathbf{n}_{i-1,j  ,k-1}\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i-1,j  ,k-1}
           \int_{\oldpartial\Omega^0} (0.5 + \xi)(0.5 - \eta)(0.5 + \zeta) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i-1,j  ,k-1}
           \int_{\oldpartial\Omega^0} (
           1 + 2\xi - 2\eta - 4\xi\eta + 2\zeta - 4\eta\zeta + 4\xi\zeta - 8 \xi\eta\zeta ) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i-1,j  ,k-1} \left(
          A_{EB} + 2 B_x - 2 B_y - 4 B_{xy} + 2 B_z - 4 B_{yz} + 4 B_{xz} - 8 B_{xyz} \right) .\\
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                       (i,j-1,k-1)                                      %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent For cell $(i,j-1,k-1)$, the basis function and its gradient are

\begin{equation*}
    \psi_{i  ,j-1,k-1} = (0.5 - \xi)(0.5 + \eta)(0.5 + \zeta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i  ,j-1,k-1} = ( 
       -(0.5 + \eta)(0.5 + \zeta)/\Delta_x, 
        (0.5 - \xi )(0.5 + \zeta)/\Delta_y,
        (0.5 - \xi )(0.5 + \eta )/\Delta_z ),
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i  ,j  }^E} U_{i  ,j-1,k-1}&\cdot(\nabla \psi_{i  ,j-1,k-1}) \; dxdydz \\
%
       &=
                    - U_x\int_{\Omega_{i  ,j-1,k-1}^0} -(0.5 + \eta)(0.5 + \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_y\int_{\Omega_{i  ,j-1,k-1}^0}  (0.5 - \xi )(0.5 + \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_v\int_{\Omega_{i  ,j-1,k-1}^0}  (0.5 - \xi )(0.5 + \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                      U_x\int_{\Omega_{i  ,j-1,k-1}^0}  (0.5 + \eta)(0.5 + \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_y\int_{\Omega_{i  ,j-1,k-1}^0}  (0.5 - \xi )(0.5 + \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_v\int_{\Omega_{i  ,j-1,k-1}^0}  (0.5 - \xi )(0.5 + \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                      U_x\int_{\Omega_{i  ,j-1,k-1}^0}  (0.25 + 0.5\eta + 0.5\zeta + \eta\zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_y\int_{\Omega_{i  ,j-1,k-1}^0}  (0.25 - 0.5\xi  + 0.5\zeta - \xi \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_v\int_{\Omega_{i  ,j-1,k-1}^0}  (0.25 - 0.5\xi  + 0.5\eta  - \xi \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%
       &=
           0.25/\Delta_x \, U_x (\Lambda + 2S_y + 2S_z + 4S_{yz})  \\
       & - 0.25/\Delta_y \, U_y (\Lambda - 2S_x + 2S_z - 4S_{xz})  \\
       & - 0.25/\Delta_z \, U_z (\Lambda - 2S_x + 2S_y - 4S_{xy})  \\
\end{align*}
The contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i  ,j-1,k-1}^E}&\psi_{i  ,j-1,k-1} \left(U_{i  ,j-1,k-1}\cdot \mathbf{n}_{i  ,j-1,k-1}\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i  ,j-1,k-1}
           \int_{\oldpartial\Omega^0} (0.5 - \xi)(0.5 + \eta)(0.5 + \zeta) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i  ,j-1,k-1}
           \int_{\oldpartial\Omega^0} (
           1 - 2\xi + 2\eta - 4\xi\eta + 2\zeta + 4\eta\zeta - 4\xi\zeta - 8 \xi\eta\zeta ) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i  ,j-1,k-1} \left(
          A_{EB} - 2 B_x + 2 B_y - 4 B_{xy} + 2 B_z + 4 B_{yz} - 4 B_{xz} - 8 B_{xyz} \right) .\\
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                        %
%                                      (i-1,j-1,k-1)                                     %
%                                                                                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent For cell $(i-1,j-1,k-1)$, the basis function and its gradient are

\begin{equation*}
    \psi_{i-1,j-1,k-1} = (0.5 + \xi)(0.5 + \eta)(0.5 + \zeta)
\end{equation*}
and
\begin{equation*}
    \nabla\psi_{i-1,j-1,k-1} = ( 
        (0.5 + \eta)(0.5 + \zeta)/\Delta_x, 
        (0.5 + \xi )(0.5 + \zeta)/\Delta_y,
        (0.5 + \xi )(0.5 + \eta )/\Delta_z ),
\end{equation*}
thus
%
\begin{align*}
     -\int_{\Omega_{i-1,j  }^E} U_{i-1,j-1,k-1}&\cdot(\nabla \psi_{i-1,j-1,k-1}) \; dxdydz \\
%
       &=
                    - U_x\int_{\Omega_{i-1,j-1,k-1}^0}  (0.5 + \eta)(0.5 + \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_y\int_{\Omega_{i-1,j-1,k-1}^0}  (0.5 + \xi )(0.5 + \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
       &\phantom{=} - U_v\int_{\Omega_{i-1,j-1,k-1}^0}  (0.5 + \xi )(0.5 + \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    - U_x\int_{\Omega_{i-1,j-1,k-1}^0}  (0.5 + \eta)(0.5 + \zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_y\int_{\Omega_{i-1,j-1,k-1}^0}  (0.5 + \xi )(0.5 + \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_v\int_{\Omega_{i-1,j-1,k-1}^0}  (0.5 + \xi )(0.5 + \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%%
%       &=
%                    - U_x\int_{\Omega_{i-1,j-1,k-1}^0}  (0.25 + 0.5\eta + 0.5\zeta + \eta\zeta)/\Delta_x \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_y\int_{\Omega_{i-1,j-1,k-1}^0}  (0.25 + 0.5\xi  + 0.5\zeta + \xi \zeta)/\Delta_y \; d\xi d\eta d\zeta \\
%       &\phantom{=} - U_v\int_{\Omega_{i-1,j-1,k-1}^0}  (0.25 + 0.5\xi  + 0.5\eta  + \xi \eta )/\Delta_z \; d\xi d\eta d\zeta \\
%
       &=
         - 0.25/\Delta_x \, U_x (\Lambda + 2S_y + 2S_z + 4S_{yz})  \\
       & - 0.25/\Delta_y \, U_y (\Lambda + 2S_x + 2S_z + 4S_{xz})  \\
       & - 0.25/\Delta_z \, U_z (\Lambda + 2S_x + 2S_y + 4S_{xy})  \\
\end{align*}
The contribution from the embedded boundary,
\begin{align*}
     \int_{\oldpartial\Omega_{i-1,j-1,k-1}^E}&\psi_{i-1,j-1,k-1} \left(U_{i-1,j-1,k-1}\cdot \mathbf{n}_{i-1,j-1,k-1}\right) \; ds \\
%
       &= \left(U\cdot \mathbf{n}\right)_{i-1,j-1,k-1}
           \int_{\oldpartial\Omega^0} (0.5 + \xi)(0.5 + \eta)(0.5 + \zeta) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i-1,j-1,k-1}
           \int_{\oldpartial\Omega^0} (
           1 + 2\xi + 2\eta + 4\xi\eta + 2\zeta + 4\eta\zeta + 4\xi\zeta + 8 \xi\eta\zeta ) \; ds \\
%
       &= 0.125 \left(U\cdot \mathbf{n}\right)_{i-1,j-1,k-1} \left(
          A_{EB} + 2 B_x + 2 B_y + 4 B_{xy} + 2 B_z + 4 B_{yz} + 4 B_{xz} + 8 B_{xyz} \right) .\\
\end{align*}

\noindent Summing all the terms, we get
%%%%\begin{equation*}
%%%%\begin{split}
%%%%     -\int U \cdot(\nabla \psi) \; dV  &= \\
%%%%%
%%%%       &0.5/\Delta_x  \big(
%%%%       - u_{i-1,j-1            } \left( \Lambda_{i-1,j-1            } + 2 S_{y_{i-1,j-1            }} \right)
%%%%       + u_{i  ,j-1            } \left( \Lambda_{i  ,j-1            } + 2 S_{y_{i  ,j-1            }} \right) \\  
%%%%       &\phantom{0.5\Delta_x\big(\;\;}
%%%%       - u_{i-1,j  \phantom{-1}} \left( \Lambda_{i-1,j  \phantom{-1}} - 2 S_{y_{i-1,j  \phantom{-1}}} \right) 
%%%%       + u_{i  ,j  \phantom{-1}} \left( \Lambda_{i  ,j  \phantom{-1}} - 2 S_{y_{i  ,j  \phantom{-1}}} \right) \big) \\
%%%%%
%%%%      + &0.5/\Delta_y \big( 
%%%%       - v_{i-1,j-1            } \left( \Lambda_{i-1,j-1            } + 2 S_{x_{i-1,j-1            }} \right)
%%%%       - v_{i  ,j-1            } \left( \Lambda_{i  ,j-1            } - 2 S_{x_{i  ,j-1            }} \right) \\
%%%%       &\phantom{0.5\Delta_x\big(\;\;}
%%%%       + v_{i-1,j  \phantom{-1}} \left( \Lambda_{i-1,j  \phantom{-1}} + 2 S_{x_{i-1,j  \phantom{-1}}} \right)
%%%%       + v_{i  ,j  \phantom{-1}} \left( \Lambda_{i  ,j  \phantom{-1}} - 2 S_{x_{i  ,j  \phantom{-1}}} \right) \big) \\
%%%%%
%%%%      + &0.25 \big(
%%%%            (U_{i-1,j-1              }\cdot \mathbf{n}_{i-1,j-1              } )
%%%%                (A_{i-1,j-1} + 2 B_{x_{i-1,j-1}} 
%%%%                    + 2 B_{y_{i-1,j-1}} + 4 B_{xy_{i-1,j-1}} )\\
%%%%        &\phantom{0.25\big(}
%%%%            (U_{i  ,j-1\phantom{-1  }}\cdot \mathbf{n}_{i  ,j-1\phantom{-1  }} )
%%%%                (A_{i  ,j-1\phantom{-1  }} - 2 B_{x_{i  ,j-1\phantom{-1  }}} 
%%%%                    + 2 B_{y_{i  ,j-1\phantom{-1  }}} - 4 B_{xy_{i  ,j-1\phantom{-1  }}} )\\
%%%%        &\phantom{0.25\big(}
%%%%            (U_{i-1,j  \phantom{  -1}}\cdot \mathbf{n}_{i-1,j  \phantom{  -1}} )
%%%%                (A_{i-1,j  \phantom{  -1}} + 2 B_{x_{i-1,j  \phantom{  -1}}} 
%%%%                    - 2 B_{y_{i-1,j  \phantom{  -1}}} - 4 B_{xy_{i-1,j  \phantom{  -1}}} )\\
%%%%        &\phantom{0.25\big(}
%%%%            (U_{i  ,j  \phantom{-1-1}}\cdot \mathbf{n}_{i  ,j  \phantom{-1-1}} )
%%%%                (A_{i  ,j  \phantom{-1-1}} - 2 B_{x_{i  ,j  \phantom{-1-1}}} 
%%%%                    - 2 B_{y_{i  ,j  \phantom{-1-1}}} + 4 B_{xy_{i  ,j  \phantom{-1-1}}} ) \big)\\
%%%%\end{split}
%%%%\end{equation*}
%
\begin{equation*}
\begin{split}
     -\int U \cdot(\nabla \psi) \; dV  &= 
    -\int_{\Omega} U\cdot(\nabla \psi) \; dV + %
       \int_{\oldpartial \Omega}\psi U\cdot\mathbf{n}\; dS  \\
%
      0.25/\Delta_x  \Big( &u_{i-1,j-1,k  \phantom{    -1}} ( -\Lambda - 2S_y + 2S_z + 4S_{yz})  \\
                        +  &u_{i  ,j-1,k  \phantom{-1  -1}} ( +\Lambda + 2S_y - 2S_z - 4S_{yz})  \\
                        +  &u_{i-1,j  ,k  \phantom{  -1-1}} ( -\Lambda + 2S_y + 2S_z - 4S_{yz})  \\
                        +  &u_{i  ,j  ,k  \phantom{-1-1-1}} ( +\Lambda - 2S_y - 2S_z + 4S_{yz})  \\
                        +  &u_{i-1,j-1,k-1\phantom{      }} ( -\Lambda - 2S_y - 2S_z - 4S_{yz})  \\
                        +  &u_{i  ,j-1,k-1\phantom{-1    }} ( +\Lambda + 2S_y + 2S_z + 4S_{yz})  \\
                        +  &u_{i-1,j  ,k-1\phantom{  -1  }} ( -\Lambda + 2S_y - 2S_z + 4S_{yz})  \\
                        +  &u_{i  ,j  ,k-1\phantom{-1-1  }} ( +\Lambda - 2S_y + 2S_z - 4S_{yz}) \Big) \\
     + 0.25/\Delta_y \Big( &v_{i-1,j-1,k  \phantom{    -1}} ( -\Lambda - 2S_x + 2S_z + 4S_{xz})  \\
                        +  &v_{i  ,j-1,k  \phantom{-1  -1}} ( -\Lambda + 2S_x + 2S_z - 4S_{xz})  \\
                        +  &v_{i-1,j  ,k  \phantom{  -1-1}} ( +\Lambda + 2S_x - 2S_z - 4S_{xz})  \\
                        +  &v_{i  ,j  ,k  \phantom{-1-1-1}} ( +\Lambda - 2S_x - 2S_z + 4S_{xz})  \\
                        +  &v_{i-1,j-1,k-1\phantom{      }} ( -\Lambda - 2S_x - 2S_z - 4S_{xz})  \\
                        +  &v_{i  ,j-1,k-1\phantom{-1    }} ( -\Lambda + 2S_x - 2S_z + 4S_{xz})  \\
                        +  &v_{i-1,j  ,k-1\phantom{  -1  }} ( +\Lambda + 2S_x + 2S_z + 4S_{xz})  \\
                        +  &v_{i  ,j  ,k-1\phantom{-1-1  }} ( +\Lambda - 2S_x + 2S_z - 4S_{xz}) \Big) \\
     + 0.25/\Delta_z \Big( &w_{i-1,j-1,k  \phantom{    -1}} ( +\Lambda + 2S_x + 2S_y + 4S_{xy})  \\
                        +  &w_{i  ,j-1,k  \phantom{-1  -1}} ( +\Lambda - 2S_x + 2S_y - 4S_{xy})  \\
                        +  &w_{i-1,j  ,k  \phantom{  -1-1}} ( +\Lambda + 2S_x - 2S_y - 4S_{xy})  \\
                        +  &w_{i  ,j  ,k  \phantom{-1-1-1}} ( +\Lambda - 2S_x - 2S_y + 4S_{xy})  \\
                        +  &w_{i-1,j-1,k-1\phantom{      }} ( -\Lambda - 2S_x - 2S_y - 4S_{xy})  \\
                        +  &w_{i  ,j-1,k-1\phantom{-1    }} ( -\Lambda + 2S_x - 2S_y + 4S_{xy})  \\
                        +  &w_{i-1,j  ,k-1\phantom{  -1  }} ( -\Lambda - 2S_x + 2S_y + 4S_{xy})  \\
                        +  &w_{i  ,j  ,k-1\phantom{-1-1  }} ( -\Lambda + 2S_x + 2S_y - 4S_{xy}) \Big) \\
                          + 0.125 \Big(
           &\left(U\cdot \mathbf{n}\right)_{i-1,j-1,k  \phantom{    -1}}
               \left( A_{EB} + 2 B_x + 2 B_y + 4 B_{xy} - 2 B_z - 4 B_{yz} - 4 B_{xz} - 8 B_{xyz} \right) \\
        +  &\left(U\cdot \mathbf{n}\right)_{i  ,j-1,k  \phantom{-1  -1}}
               \left( A_{EB} - 2 B_x + 2 B_y - 4 B_{xy} - 2 B_z - 4 B_{yz} + 4 B_{xz} + 8 B_{xyz} \right) \\
        +  &\left(U\cdot \mathbf{n}\right)_{i-1,j  ,k  \phantom{  -1-1}}
               \left( A_{EB} + 2 B_x - 2 B_y - 4 B_{xy} - 2 B_z + 4 B_{yz} - 4 B_{xz} + 8 B_{xyz} \right) \\
        +  &\left(U\cdot \mathbf{n}\right)_{i  ,j  ,k  \phantom{-1-1-1}}
               \left( A_{EB} - 2 B_x - 2 B_y + 4 B_{xy} - 2 B_z + 4 B_{yz} + 4 B_{xz} - 8 B_{xyz} \right) \\
        +  &\left(U\cdot \mathbf{n}\right)_{i-1,j-1,k-1\phantom{      }}
               \left( A_{EB} + 2 B_x + 2 B_y + 4 B_{xy} + 2 B_z + 4 B_{yz} + 4 B_{xz} + 8 B_{xyz} \right) \\
        +  &\left(U\cdot \mathbf{n}\right)_{i  ,j-1,k-1\phantom{-1    }}
               \left( A_{EB} - 2 B_x + 2 B_y - 4 B_{xy} + 2 B_z + 4 B_{yz} - 4 B_{xz} - 8 B_{xyz} \right) \\
        +  &\left(U\cdot \mathbf{n}\right)_{i-1,j  ,k-1\phantom{  -1  }}
               \left( A_{EB} + 2 B_x - 2 B_y - 4 B_{xy} + 2 B_z - 4 B_{yz} + 4 B_{xz} - 8 B_{xyz} \right) \\
        +  &\left(U\cdot \mathbf{n}\right)_{i  ,j  ,k-1\phantom{-1-1  }}
               \left( A_{EB} - 2 B_x - 2 B_y + 4 B_{xy} + 2 B_z - 4 B_{yz} - 4 B_{xz} + 8 B_{xyz} \right) \Big) \\
\end{split}
\end{equation*}

\subsubsection{Computing the integrals}

\paragraph{2D Line Integrals}\mbox{} \\

In 2D we first parameterize the line segment representing the embedded boundary
\begin{equation}\label{eq:mapping:parameteric-line}
    \xi(t) = \xi_0 + (\xi_1 - \xi_0)t
    \qquad\text{and}\qquad
    \eta(t) = \eta_0 + (\eta_1 - \eta_0)t
\end{equation}
where $(\xi_0, \eta_0)$ and $(\xi_1,\eta_1)$ are the points were the boundary
intersects the unit square walls. Additionally, from the chain rule we have
\begin{equation*}
    \frac{dx}{dt} = \frac{dx}{d\xi }\frac{d\xi }{dt}
    \qquad\text{and}\qquad
    \frac{dy}{dt} = \frac{dy}{d\eta}\frac{d\eta}{dt}
\end{equation*}
where $dx/d\xi$ and $dy/d\eta$ are obtained from \eqref{eq:mapping:cell:ij}
and $d\xi/dt$ and $d\eta/dt$ are found from \eqref{eq:mapping:parameteric-line}
such that
\begin{equation}
\begin{split}
    ds &= \sqrt{ (dx)^2 + (dy)^2} \\
%       &= \sqrt{ \left(\frac{dx}{d\xi }\frac{d\xi }{dt}\right)^2 
%               + \left(\frac{dy}{d\eta}\frac{d\eta}{dt}\right)^2  } \; dt \\
%       &= \sqrt{ \left(\Delta_x\frac{d\xi }{dt}\right)^2 
%               + \left(\Delta_y\frac{d\eta}{dt}\right)^2  } \; dt \\
       &= \sqrt{ \left(\Delta_x(\xi_1  - \xi_0 )\right)^2 
               + \left(\Delta_y(\eta_1 - \eta_0)\right)^2  } \; dt
\end{split}
\end{equation}
If $\Delta_x = \Delta_y$, then we can further simplify this expression.%

\begin{equation*}
    ds = \Delta_x\sqrt{(\xi_1 - \xi_0)^2 + (\eta_1 - \eta_0)^2} dt
\end{equation*}
Now to compute the integrals,
\begin{equation}
\begin{split}
    A_{i,j} &= \int_{\oldpartial\Omega^0} 1 ds \\
      &= \int_0^1
        \sqrt{ \left(\Delta_x(\xi_1  - \xi_0 )\right)^2 
               + \left(\Delta_y(\eta_1 - \eta_0)\right)^2  } \; dt \\
      &= \sqrt{ \left(\Delta_x(\xi_1  - \xi_0 )\right)^2 
              + \left(\Delta_y(\eta_1 - \eta_0)\right)^2  } \\
\end{split}
\end{equation}


\begin{equation}
\begin{split}
    B_x &= \int_{\oldpartial\Omega^0} \xi ds \\
        &= A_{i,j} \int_0^1 (\xi_0 + (\xi_1 - \xi_0)t)  \; dt \\
        &= A_{i,j} \frac{\xi_1 + \xi_0}{2} \\
\end{split}
\end{equation}


\begin{equation}
\begin{split}
    B_y &= \int_{\oldpartial\Omega^0} \eta ds \\
        &= A_{i,j} \int_0^1 (\eta_0 + (\eta_1 - \eta_0)t) \; dt \\
        &= A_{i,j} \frac{\eta_1 + \eta_0}{2} \\
\end{split}
\end{equation}


\begin{equation}
\begin{split}
    B_{xy} &= \int_{\oldpartial\Omega^0} \xi\eta ds \\
        &= A_{i,j} \int_0^1
           \Big(
               \xi_0\eta_0
               + \left( \xi_0(\eta_1 - \eta_0) + \eta_0(\xi_1 - \xi_0\right) t
               + \left( \xi_1 - \xi_0)(\eta_1 - \eta_0 \right) t^2
           \Big)  \; dt \\
        &= A_{i,j} \Big(
               \xi_0\eta_0
               + \frac{1}{2} \left( \xi_0(\eta_1 - \eta_0) + \eta_0(\xi_1 - \xi_0\right) 
               + \frac{1}{3} \left( \xi_1 - \xi_0)(\eta_1 - \eta_0 \right)
           \Big) \\
\end{split}
\end{equation}


\paragraph{3D Surface Integrals}\mbox{} \\

The surface integrals for 3D are computed by using code from ALGOIM \cite{algoim} customized for AMReX's geometry methodology.


==> EB-Flow/nodal-mapping.tex <==
\begin{tikzpicture} [scale=1.2]

\coordinate (n00) at (2,2);
\coordinate (n10) at (4,2);
\coordinate (n11) at (4,4);
\coordinate (n01) at (2,4);

\fill[blue!10] (n00) rectangle (n11);

\coordinate (LL) at (0,0);
\coordinate (UR) at (4,4);

\draw[step=2,gray,very thin] (LL) grid (UR);


\foreach \lj in {0.5,2.5} {
  \foreach \li in {0.5,2.5} {
    \draw[blue!75, -{Triangle[width=4pt,length=3pt]}, line width=0.5pt] 
        ({\li+0.29}, {\lj+0.50}) -- ({\li+0.73}, {\lj+0.50});
    \draw[red!75, -{Triangle[width=4pt,length=3pt]}, line width=0.5pt] 
        ({\li+0.50}, {\lj+0.29}) -- ({\li+0.50}, {\lj+0.73});
    \fill[black] ({\li+0.5},{\lj+0.5}) circle [radius=1.15pt];
  }
}

\foreach \lj in {0,2,4} {
  \foreach \li in {0,2,4} {
    \ifthenelse{\({\li}=1 \AND {\lj}=1\)}{
    \draw ({\li},{\lj}) circle [radius=1.5pt];
    }{
    \fill[gray!40] ({\li},{\lj}) circle [radius=1.5pt];
    }
  }
}

% Labels
%\draw (n00) node [below] {\scriptsize{$(x_{i  ,j  },y_{i  ,j  })$}};
%\draw (n10) node [below] {\scriptsize{$(x_{i+1,j  },y_{i+1,j  })$}};
%\draw (n11) node [above] {\scriptsize{$(x_{i+1,j+1},y_{i+1,j+1})$}};
%\draw (n01) node [above] {\scriptsize{$(x_{i  ,j+1},y_{i  ,j+1})$}};
\draw (n00) node [below] {\scriptsize{$(x_{i  },y_{j  })$}};
\draw (n10) node [below] {\scriptsize{$(x_{i+1},y_{j  })$}};
\draw (n11) node [above] {\scriptsize{$(x_{i+1},y_{j+1})$}};
\draw (n01) node [above] {\scriptsize{$(x_{i  },y_{j+1})$}};

\draw (1.0,0) node [below]  {\scriptsize{$i-1$}};
\draw (3.0,0) node [below]  {\scriptsize{$i$}};

\draw (0,1.0) node [left]  {\scriptsize{$j-1$}};
\draw (0,3.0) node [left]  {\scriptsize{$j$}};

\end{tikzpicture}
